MMTEB: Massive Multilingual Text Embedding Benchmark

Text embeddings are typically evaluated on a limited set of tasks, which are constrained by language, domain, and task diversity. To address these limitations and provide a more comprehensive evaluation, we introduce the Massive Multilingual Text Embedding Benchmark (MMTEB) - a large-scale, community-driven expansion of MTEB, covering over 500 quality-controlled evaluation tasks across 250+ languages. MMTEB includes a diverse set of challenging, novel tasks such as instruction following, long-document retrieval, and code retrieval, representing the largest multilingual collection of evaluation tasks for embedding models to date. Using this collection, we develop several highly multilingual benchmarks, which we use to evaluate a representative set of models. We find that while large language models (LLMs) with billions of parameters can achieve state-of-the-art performance on certain language subsets and task categories, the best-performing publicly available model is multilingual-e5-large-instruct with only 560 million parameters. To facilitate accessibility and reduce computational cost, we introduce a novel downsampling method based on inter-task correlation, ensuring a diverse selection while preserving relative model rankings. Furthermore, we optimize tasks such as retrieval by sampling hard negatives, creating smaller but effective splits. These optimizations allow us to introduce benchmarks that drastically reduce computational demands. For instance, our newly introduced zero-shot English benchmark maintains a ranking order similar to the full-scale version but at a fraction of the computational cost.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/09-Acknowledgements.tex <==
\subsubsection*{Acknowledgments}
% adds acknowledgement of contributors which were not co-authors
% acknowledgement on compute resources given
% other?

==> tables/tasks.tex <==
\fontsize{9}{11}\selectfont
\onecolumn
\setlength\extrarowheight{7pt}
\begin{longtable}{L{5.0cm}|L{1.5cm}L{1.4cm}L{1.4cm}L{1.4cm}L{1.4cm}L{1.0cm}L{1.0cm}}
\toprule
\textbf{Dataset} & \textbf{N Langs} & \textbf{Type} & \textbf{Category} & \textbf{Domains} & \textbf{N Docs} & 
\textbf{Avg. Length} \\ 
\midrule
\endhead \\AFQMC \cite{raghu-etal-2021-end} & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
AILACasedocs \cite{paheli_bhattacharya_2020_4063986} & 1 (eng) & Retrieval & p2p & Legal &  &  \\
 \hline 
AILAStatutes \cite{paheli_bhattacharya_2020_4063986} & 1 (eng) & Retrieval & p2p & Legal &  &  \\
 \hline 
AJGT \cite{alomari2017arabic} & 1 (ara) & Classification & s2s & Social & 1800.0 & 46.8 \\
 \hline 
ARCChallenge \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 1172.0 & 161.7 \\
 \hline 
ATEC \cite{raghu-etal-2021-end} & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
AfriSentiClassification \cite{Muhammad2023AfriSentiAT} & 12 (amh, arq, ary, hau, ibo, kin, pcm, por, swa, tso, twi...) & Classification & s2s & Social & 2048.0 & 74.8 \\
 \hline 
AfriSentiLangClassification  & 12 (amh, arq, ary, hau, ibo, kin, pcm, por, swa, tso, twi...) & Classification & s2s & Social & 5754.0 & 77.8 \\
 \hline 
AllegroReviews  & 1 (pol) & Classification & s2s &  & 1006.0 & 477.2 \\
 \hline 
AlloProfClusteringP2P.v2 \cite{lef23} & 1 (fra) & Clustering & p2p & Encyclopaedic & 2556.0 & 3539.5 \\
 \hline 
AlloProfClusteringS2S.v2 \cite{lef23} & 1 (fra) & Clustering & s2s & Encyclopaedic & 2556.0 & 32.8 \\
 \hline 
AlloprofReranking \cite{lef23} & 1 (fra) & Reranking & s2p & Web, Academic & 5790.0 &  \\
 \hline 
AlloprofRetrieval \cite{lef23} & 1 (fra) & Retrieval & s2p & Encyclopaedic & 2048.0 &  \\
 \hline 
AlphaNLI \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 1532.0 & 147.8 \\
 \hline 
AmazonCounterfactualClassification \cite{oneill-etal-2021-wish} & 3 (deu, eng, jpn) & Classification & s2s & Reviews & 502.5 & 107.7 \\
 \hline 
AmazonPolarityClassification \cite{McAuley2013HiddenFA} & 1 (eng) & Classification & s2s & Reviews & 400000.0 & 431.4 \\
 \hline 
AmazonReviewsClassification \cite{keung2020multilingual} & 6 (cmn, deu, eng, fra, jpn, spa) & Classification & s2s & Reviews & 30000.0 & 159.8 \\
 \hline 
AngryTweetsClassification \cite{pauli2021danlp} & 1 (dan) & Classification & s2s & Social & 1050.0 & 156.1 \\
 \hline 
ArEntail \cite{obeidat2024arentail} & 1 (ara) & PairClassification & s2s & News & 1000.0 & 65.8 \\
 \hline 
ArXivHierarchicalClusteringP2P \cite{arXiv.org e-Print archive} & 1 (eng) & Clustering & p2p & Academic & 2048.0 & 1010.0 \\
 \hline 
ArXivHierarchicalClusteringS2S \cite{arXiv.org e-Print archive} & 1 (eng) & Clustering & p2p & Academic & 2048.0 & 1010.0 \\
 \hline 
ArguAna \cite{boteva2016} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
ArguAna-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
ArmenianParaphrasePC \cite{malajyan2020arpa} & 1 (hye) & PairClassification & s2s & News & 2746.5 & 242.6 \\
 \hline 
ArxivClassification \cite{8675939} & 1 (eng) & Classification & s2s & Academic & 2048.0 &  \\
 \hline 
AskUbuntuDupQuestions \cite{wang-2021-TSDAE} & 1 (eng) & Reranking & s2s &  & 2255.0 & 52.5 \\
 \hline 
Assin2RTE \cite{real2020assin} & 1 (por) & PairClassification & s2s &  & 2448.0 & 53.5 \\
 \hline 
Assin2STS \cite{real2020assin} & 1 (por) & STS & s2s &  & 2448.0 & 53.5 \\
 \hline 
BIOSSES \cite{10.1093/bioinformatics/btx238} & 1 (eng) & STS & s2s &  &  &  \\
 \hline 
BQ \cite{raghu-etal-2021-end} & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
BSARDRetrieval \cite{louis2022statutory} & 1 (fra) & Retrieval & s2p & Legal & 222.0 & 71.9 \\
 \hline 
BUCC.v2 \cite{zweigenbaum-etal-2017-overview} & 5 (cmn, deu, eng, fra, rus) & BitextMining & s2s &  & 641684.0 & 101.3 \\
 \hline 
Banking77Classification \cite{casanueva-etal-2020-efficient} & 1 (eng) & Classification & s2s &  & 3080.0 & 54.2 \\
 \hline 
BelebeleRetrieval \cite{bandarkar2023belebele} & 115 (acm, afr, als, amh, apc, arb, ars, ary, arz, asm, azj...) & Retrieval & s2p & Web, News & 103500.0 & 568.0 \\
 \hline 
BengaliDocumentClassification \cite{akash-etal-2023-shironaam} & 1 (ben) & Classification & s2s & News & 2048.0 & 1658.1 \\
 \hline 
BengaliHateSpeechClassification \cite{karim2020BengaliNLP} & 1 (ben) & Classification & s2s & News & 3418.0 & 103.4 \\
 \hline 
BengaliSentimentAnalysis \cite{sazzed2020cross} & 1 (ben) & Classification & s2s & Reviews & 11807.0 & 69.7 \\
 \hline 
BibleNLPBitextMining \cite{akerman2023ebible} & 829 (aai, aak, aau, aaz, abt, abx, aby, acf, acr, acu, adz...) & BitextMining & s2s & Religious & 256.0 & 120.0 \\
 \hline 
BigPatentClustering.v2 \cite{DBLP:journals/corr/abs-1906-03741} & 1 (eng) & Clustering & p2p & Legal & 2048.0 & 30995.5 \\
 \hline 
BiorxivClusteringP2P.v2  & 1 (eng) & Clustering & p2p & Academic & 2048.0 & 1664.0 \\
 \hline 
BiorxivClusteringS2S.v2  & 1 (eng) & Clustering & s2s & Academic & 2048.0 & 101.7 \\
 \hline 
BlurbsClusteringP2P.v2 \cite{Remus2019GermEval2T} & 1 (deu) & Clustering & p2p & Fiction & 2048.0 & 664.1 \\
 \hline 
BlurbsClusteringS2S.v2 \cite{Remus2019GermEval2T} & 1 (deu) & Clustering & s2s & Fiction & 2048.0 & 23.0 \\
 \hline 
BornholmBitextMining \cite{derczynskiBornholmskNaturalLanguage2019} & 1 (dan) & BitextMining & s2s & Web, Social, Fiction & 500.0 & 89.7 \\
 \hline 
BrazilianToxicTweetsClassification \cite{DBLP:journals/corr/abs-2010-04543} & 1 (por) & MultilabelClassification & s2s & Constructed & 2048.0 & 85.0 \\
 \hline 
BulgarianStoreReviewSentimentClassfication \cite{DVN/TXIK9P_2018} & 1 (bul) & Classification & s2s & Reviews & 182.0 & 316.7 \\
 \hline 
CBD \cite{ogr:kob:19:poleval} & 1 (pol) & Classification & s2s &  & 1000.0 & 93.2 \\
 \hline 
CDSC-E \cite{wroblewska-krasnowska-kieras-2017-polish} & 1 (pol) & PairClassification & s2s &  &  &  \\
 \hline 
CDSC-R \cite{wroblewska-krasnowska-kieras-2017-polish} & 1 (pol) & STS & s2s & Web & 1000.0 & 75.2 \\
 \hline 
CEDRClassification \cite{sboev2021data} & 1 (rus) & MultilabelClassification & s2s & Web, Social, Blog & 1882.0 & 91.2 \\
 \hline 
CLSClusteringP2P.v2 \cite{li2022csl} & 1 (cmn) & Clustering & p2p & Academic & 2048.0 &  \\
 \hline 
CLSClusteringS2S.v2 \cite{li2022csl} & 1 (cmn) & Clustering & s2s & Academic & 2048.0 &  \\
 \hline 
CMedQAv1-reranking \cite{zhang2017chinese} & 1 (cmn) & Reranking & s2s & Medical & 2000.0 & 165.0 \\
 \hline 
CMedQAv2-reranking \cite{8548603} & 1 (cmn) & Reranking & s2s &  &  &  \\
 \hline 
CQADupstackAndroidRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackEnglishRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackGamingRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackGisRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackMathematicaRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackPhysicsRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackProgrammersRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackStatsRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackTexRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackUnixRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackWebmastersRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CQADupstackWordpressRetrieval \cite{hoogeveen2015} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CSFDCZMovieReviewSentimentClassification \cite{štefánik2023resources} & 1 (ces) & Classification & s2s & Reviews & 2048.0 & 386.5 \\
 \hline 
CSFDSKMovieReviewSentimentClassification \cite{štefánik2023resources} & 1 (slk) & Classification & s2s & Reviews & 2048.0 & 366.2 \\
 \hline 
CTKFactsNLI \cite{ullrich2023csfever} & 1 (ces) & PairClassification & s2s & News & 340.0 & 222.5 \\
 \hline 
CUADAffiliateLicenseLicenseeLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 198.0 & 484.1 \\
 \hline 
CUADAffiliateLicenseLicensorLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 88.0 & 633.4 \\
 \hline 
CUADAntiAssignmentLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1172.0 & 340.8 \\
 \hline 
CUADAuditRightsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1216.0 & 337.1 \\
 \hline 
CUADCapOnLiabilityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1246.0 & 375.7 \\
 \hline 
CUADChangeOfControlLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 416.0 & 392.0 \\
 \hline 
CUADCompetitiveRestrictionExceptionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 220.0 & 433.0 \\
 \hline 
CUADCovenantNotToSueLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 308.0 & 403.0 \\
 \hline 
CUADEffectiveDateLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 236.0 & 277.6 \\
 \hline 
CUADExclusivityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 762.0 & 369.2 \\
 \hline 
CUADExpirationDateLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 876.0 & 309.3 \\
 \hline 
CUADGoverningLawLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 876.0 & 289.9 \\
 \hline 
CUADIPOwnershipAssignmentLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 576.0 & 414.0 \\
 \hline 
CUADInsuranceLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1030.0 & 365.5 \\
 \hline 
CUADIrrevocableOrPerpetualLicenseLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 280.0 & 473.4 \\
 \hline 
CUADJointIPOwnershipLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 192.0 & 374.2 \\
 \hline 
CUADLicenseGrantLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1396.0 & 409.9 \\
 \hline 
CUADLiquidatedDamagesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 220.0 & 351.8 \\
 \hline 
CUADMinimumCommitmentLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 772.0 & 364.2 \\
 \hline 
CUADMostFavoredNationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 64.0 & 418.8 \\
 \hline 
CUADNoSolicitOfCustomersLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 84.0 & 392.9 \\
 \hline 
CUADNoSolicitOfEmployeesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 142.0 & 417.9 \\
 \hline 
CUADNonCompeteLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 442.0 & 383.2 \\
 \hline 
CUADNonDisparagementLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 100.0 & 403.1 \\
 \hline 
CUADNonTransferableLicenseLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 542.0 & 399.2 \\
 \hline 
CUADNoticePeriodToTerminateRenewalLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 222.0 & 354.9 \\
 \hline 
CUADPostTerminationServicesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 808.0 & 422.5 \\
 \hline 
CUADPriceRestrictionsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 46.0 & 324.7 \\
 \hline 
CUADRenewalTermLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 386.0 & 340.9 \\
 \hline 
CUADRevenueProfitSharingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 774.0 & 371.6 \\
 \hline 
CUADRofrRofoRofnLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 690.0 & 395.5 \\
 \hline 
CUADSourceCodeEscrowLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 118.0 & 399.2 \\
 \hline 
CUADTerminationForConvenienceLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 430.0 & 326.3 \\
 \hline 
CUADThirdPartyBeneficiaryLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 68.0 & 261.0 \\
 \hline 
CUADUncappedLiabilityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 294.0 & 441.0 \\
 \hline 
CUADUnlimitedAllYouCanEatLicenseLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 48.0 & 368.1 \\
 \hline 
CUADVolumeRestrictionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 322.0 & 306.3 \\
 \hline 
CUADWarrantyDurationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 320.0 & 352.3 \\
 \hline 
CanadaTaxCourtOutcomesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 244.0 & 622.6 \\
 \hline 
CataloniaTweetClassification \cite{zotova-etal-2020-multilingual} & 2 (cat, spa) & Classification & s2s & Social, Government & 2000.0 & 201.6 \\
 \hline 
ClimateFEVER \cite{diggelmann2021climatefever} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
CmedqaRetrieval  & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
Cmnli \cite{xu-etal-2020-clue} & 1 (cmn) & PairClassification & s2s &  &  &  \\
 \hline 
CodeEditSearchRetrieval \cite{muennighoff2023octopack} & 13 (c, c++, go, java, javascript, php, python, ruby, rust, scala, shell...) & Retrieval & p2p & Programming & 13000.0 & 553.5 \\
 \hline 
CodeSearchNetRetrieval \cite{husain2019codesearchnet} & 6 (go, java, javascript, php, python, ruby) & Retrieval & p2p & Programming & 1000.0 & 1196.5 \\
 \hline 
ContractNLIConfidentialityOfAgreementLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 82.0 & 473.2 \\
 \hline 
ContractNLIExplicitIdentificationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 109.0 & 506.1 \\
 \hline 
ContractNLIInclusionOfVerballyConveyedInformationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 139.0 & 525.8 \\
 \hline 
ContractNLILimitedUseLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 208.0 & 407.5 \\
 \hline 
ContractNLINoLicensingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 162.0 & 419.4 \\
 \hline 
ContractNLINoticeOnCompelledDisclosureLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 142.0 & 503.4 \\
 \hline 
ContractNLIPermissibleAcquirementOfSimilarInformationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 178.0 & 427.4 \\
 \hline 
ContractNLIPermissibleCopyLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 87.0 & 386.8 \\
 \hline 
ContractNLIPermissibleDevelopmentOfSimilarInformationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 136.0 & 396.4 \\
 \hline 
ContractNLIPermissiblePostAgreementPossessionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 111.0 & 529.1 \\
 \hline 
ContractNLIReturnOfConfidentialInformationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 66.0 & 478.3 \\
 \hline 
ContractNLISharingWithEmployeesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 170.0 & 548.6 \\
 \hline 
ContractNLISharingWithThirdPartiesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 180.0 & 517.3 \\
 \hline 
ContractNLISurvivalOfObligationsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 157.0 & 417.6 \\
 \hline 
Core17InstructionRetrieval \cite{weller2024followir} & 1 (eng) & InstructionRetrieval & s2p & News & 39838.0 & 2768.7 \\
 \hline 
CorporateLobbyingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 490.0 & 6039.9 \\
 \hline 
CovidRetrieval  & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
CrossLingualSemanticDiscriminationWMT19  & 2 (deu, fra) & Retrieval & s2s & News & 2946.0 & 161.0 \\
 \hline 
CrossLingualSemanticDiscriminationWMT21  & 2 (deu, fra) & Retrieval & s2s & News & 1786.0 & 159.0 \\
 \hline 
CyrillicTurkicLangClassification \cite{goldhahn2012building} & 9 (bak, chv, kaz, kir, krc, rus, sah, tat, tyv) & Classification & s2s & Web & 2048.0 & 92.2 \\
 \hline 
CzechProductReviewSentimentClassification \cite{habernal-etal-2013-sentiment} & 1 (ces) & Classification & s2s & Reviews & 2048.0 & 153.3 \\
 \hline 
CzechSoMeSentimentClassification \cite{habernal-etal-2013-sentiment} & 1 (ces) & Classification & s2s & Reviews & 1000.0 & 59.9 \\
 \hline 
CzechSubjectivityClassification \cite{priban-steinberger-2022-czech} & 1 (ces) & Classification & s2s & Reviews & 1250.0 & 108.2 \\
 \hline 
DBPedia \cite{Hasibi:2017:DVT} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
DBPedia-PL \cite{Hasibi:2017:DVT} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
DBpediaClassification \cite{NIPS2015_250cf8b5} & 1 (eng) & Classification & s2s & Encyclopaedic & 70000.0 & 281.4 \\
 \hline 
DKHateClassification \cite{sigurbergsson-derczynski-2020-offensive} & 1 (dan) & Classification & s2s & Social & 329.0 & 104.0 \\
 \hline 
DalajClassification \cite{2105.06681} & 1 (swe) & Classification & s2s & Non-fiction & 444.0 & 243.8 \\
 \hline 
DanFEVER \cite{norregaard-derczynski-2021-danfever} & 1 (dan) & Retrieval & p2p & Encyclopaedic, Non-fiction & 8897.0 & 124.8 \\
 \hline 
DanishPoliticalCommentsClassification \cite{SAMsentiment} & 1 (dan) & Classification & s2s & Social & 9010.0 & 69.9 \\
 \hline 
DefinitionClassificationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1337.0 & 253.7 \\
 \hline 
DiaBlaBitextMining \cite{gonzalez2019diabla} & 2 (eng, fra) & BitextMining & s2s & Social &  &  \\
 \hline 
Diversity1LegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 300.0 & 103.2 \\
 \hline 
Diversity2LegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 300.0 & 0.0 \\
 \hline 
Diversity3LegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 300.0 & 135.5 \\
 \hline 
Diversity4LegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 300.0 & 144.5 \\
 \hline 
Diversity5LegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 300.0 & 174.8 \\
 \hline 
Diversity6LegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 300.0 & 301.0 \\
 \hline 
DuRetrieval \cite{qiu2022dureaderretrieval} & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
DutchBookReviewSentimentClassification \cite{DBLP:journals/corr/abs-1910-00896} & 1 (nld) & Classification & s2s & Reviews & 2224.0 & 1443.0 \\
 \hline 
EcomRetrieval  & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
EightTagsClustering.v2 \cite{dadas-etal-2020-evaluation} & 1 (pol) & Clustering & s2s & Social & 2048.0 & 78.7 \\
 \hline 
EmotionClassification \cite{saravia-etal-2018-carer} & 1 (eng) & Classification & s2s & Social & 2000.0 & 95.4 \\
 \hline 
EstQA \cite{mastersthesis} & 1 (est) & Retrieval & s2p & Encyclopaedic & 603.0 & 772.5 \\
 \hline 
EstonianValenceClassification \cite{Pajupuu2023} & 1 (est) & Classification & s2s & News & 2044.0 & 229.1 \\
 \hline 
FEVER \cite{thorne-etal-2018-fever} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
FQuADRetrieval \cite{dhoffschmidt-etal-2020-fquad} & 1 (fra) & Retrieval & s2p & Encyclopaedic & 250.0 & 933.5 \\
 \hline 
FaithDial \cite{dziri2022faithdial} & 1 (eng) & Retrieval & s2p & Encyclopaedic & 2042.0 & 74.0 \\
 \hline 
FalseFriendsGermanEnglish \cite{Chibb_2022} & 1 (deu) & PairClassification & s2s &  & 1524.0 & 40.3 \\
 \hline 
FaroeseSTS \cite{snaebjarnarson-etal-2023-transfer} & 1 (fao) & STS & s2s & News, Web & 729.0 & 43.6 \\
 \hline 
FarsTail \cite{amirkhani2023farstail} & 1 (fas) & PairClassification & s2s & Academic & 1029.0 & 125.8 \\
 \hline 
FeedbackQARetrieval \cite{li-etal-2022-using} & 1 (eng) & Retrieval & s2p & Web, Government, Medical & 1992.0 & 1175.0 \\
 \hline 
FiQA-PL \cite{thakur2021beir} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
FiQA2018 \cite{thakur2021beir} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
FilipinoHateSpeechClassification \cite{Cabasag-2019-hate-speech} & 1 (fil) & Classification & s2s & Social & 2048.0 & 87.8 \\
 \hline 
FilipinoShopeeReviewsClassification \cite{riegoenhancement} & 1 (fil) & Classification & s2s & Social & 2250.0 & 144.4 \\
 \hline 
FinParaSTS \cite{kanerva-etal-2021-finnish} & 1 (fin) & STS & s2s & News, Subtitles & 1000.0 & 58.9 \\
 \hline 
FinToxicityClassification \cite{eskelinen-etal-2023-toxicity} & 1 (fin) & Classification & s2s & News & 2048.0 & 416.8 \\
 \hline 
FinancialPhrasebankClassification \cite{Malo2014GoodDO} & 1 (eng) & Classification & s2s & News & 4840.0 & 122.0 \\
 \hline 
FloresBitextMining \cite{goyal2022flores} & 196 (ace, acm, acq, aeb, afr, ajp, aka, als, amh, apc, arb...) & BitextMining & s2s & Non-fiction, Encyclopaedic & 1004.5 &  \\
 \hline 
FrenchBookReviews  & 1 (fra) & Classification & s2s & Reviews & 2048.0 & 311.5 \\
 \hline 
FrenkEnClassification \cite{ljubešić2019frenk} & 1 (eng) & Classification & s2s & Social & 2300.0 & 188.8 \\
 \hline 
FrenkHrClassification \cite{ljubešić2019frenk} & 1 (hrv) & Classification & s2s & Social & 2120.0 & 89.9 \\
 \hline 
FrenkSlClassification \cite{ljubešić2019frenk} & 1 (slv) & Classification & s2s & Social & 2177.0 & 136.6 \\
 \hline 
FunctionOfDecisionSectionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 367.0 & 551.1 \\
 \hline 
GeoreviewClassification  & 1 (rus) & Classification & p2p & Reviews & 2048.0 & 409.0 \\
 \hline 
GeoreviewClusteringP2P  & 1 (rus) & Clustering & p2p & Reviews & 2000.0 & 384.5 \\
 \hline 
GeorgianFAQRetrieval  & 1 (kat) & Retrieval & s2p & Web & 2566.0 & 572.0 \\
 \hline 
GerDaLIR \cite{wrzalik-krechel-2021-gerdalir} & 1 (deu) & Retrieval & s2p &  &  &  \\
 \hline 
GerDaLIRSmall \cite{wrzalik-krechel-2021-gerdalir} & 1 (deu) & Retrieval & p2p & Legal &  &  \\
 \hline 
GermanDPR \cite{möller2021germanquad} & 1 (deu) & Retrieval & s2p &  &  &  \\
 \hline 
GermanGovServiceRetrieval \cite{lhm-dienstleistungen-qa} & 1 (deu) & Retrieval & s2p & Government & 357.0 & 1211.7 \\
 \hline 
GermanPoliticiansTwitterSentimentClassification \cite{schmidt-etal-2022-sentiment} & 1 (deu) & Classification & s2s & Social, Government & 357.0 & 302.5 \\
 \hline 
GermanQuAD-Retrieval  & 1 (deu) & Retrieval & s2p &  &  &  \\
 \hline 
GermanSTSBenchmark \cite{huggingface:dataset:stsb_multi_mt} & 1 (deu) & STS & s2s &  &  &  \\
 \hline 
GreekCivicsQA  & 1 (ell) & Retrieval & s2p & Academic & 407.0 & 2226.8 \\
 \hline 
GreekLegalCodeClassification \cite{papaloukas-etal-2021-glc} & 1 (ell) & Classification & s2s & Legal & 2048.0 & 4123.8 \\
 \hline 
GujaratiNewsClassification  & 1 (guj) & Classification & s2s & News & 3293.5 & 61.9 \\
 \hline 
HALClusteringS2S.v2 \cite{ciancone2024extending} & 1 (fra) & Clustering & s2s & Academic & 2048.0 & 86.6 \\
 \hline 
HagridRetrieval \cite{hagrid} & 1 (eng) & Retrieval & s2p & Encyclopaedic & 1922.0 & 14.5 \\
 \hline 
HateSpeechPortugueseClassification \cite{fortuna-etal-2019-hierarchically} & 1 (por) & Classification & s2s & Social & 2048.0 & 101.0 \\
 \hline 
HeadlineClassification \cite{gudkov-etal-2020-automatically} & 1 (rus) & Classification & s2s & News & 2048.0 & 61.6 \\
 \hline 
HebrewSentimentAnalysis \cite{amram-etal-2018-representations} & 1 (heb) & Classification & s2s & Reviews & 2048.0 & 113.6 \\
 \hline 
HellaSwag \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 10042.0 & 366.1 \\
 \hline 
HinDialectClassification \cite{11234/1-4839} & 21 (anp, awa, ben, bgc, bhb, bhd, bho, bjj, bns, bra, gbm...) & Classification & s2s & Social, Spoken & 1152.0 & 583.8 \\
 \hline 
HindiDiscourseClassification \cite{dhanwal-etal-2020-annotated} & 1 (hin) & Classification & s2s & Fiction, Social & 2048.0 & 79.2 \\
 \hline 
HotelReviewSentimentClassification \cite{elnagar2018hotel} & 1 (ara) & Classification & s2s & Reviews & 2048.0 & 137.2 \\
 \hline 
HotpotQA \cite{yang-etal-2018-hotpotqa} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
HotpotQA-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
HunSum2AbstractiveRetrieval \cite{barta2024news} & 1 (hun) & Retrieval & s2p & News & 1998.0 & 2462.2 \\
 \hline 
IFlyTek \cite{xu-etal-2020-clue} & 1 (cmn) & Classification & s2s &  &  &  \\
 \hline 
IN22ConvBitextMining \cite{gala2023indictrans} & 23 (asm, ben, brx, doi, eng, gom, guj, hin, kan, kas, mai...) & BitextMining & s2s & Social, Spoken, Fiction & 1503.0 & 54.3 \\
 \hline 
IN22GenBitextMining \cite{gala2023indictrans} & 23 (asm, ben, brx, doi, eng, gom, guj, hin, kan, kas, mai...) & BitextMining & s2s & Web, Legal, Government, News, Religious, Non-fiction & 1024.0 & 156.7 \\
 \hline 
IWSLT2017BitextMining \cite{cettolo-etal-2017-overview} & 10 (ara, cmn, deu, eng, fra, ita, jpn, kor, nld, ron) & BitextMining & s2s & Non-fiction, Fiction & 21928.0 & 95.4 \\
 \hline 
ImdbClassification \cite{maas-etal-2011-learning} & 1 (eng) & Classification & p2p & Reviews & 25000.0 & 1293.8 \\
 \hline 
InappropriatenessClassification \cite{babakov-etal-2021-detecting} & 1 (rus) & Classification & s2s & Web, Social & 2048.0 & 97.7 \\
 \hline 
IndicCrosslingualSTS \cite{10.1162/tacl_a_00452} & 13 (asm, ben, eng, guj, hin, kan, mal, mar, ory, pan, tam...) & STS & s2s & News, Non-fiction, Web, Spoken, Government & 10020.0 & 76.2 \\
 \hline 
IndicGenBenchFloresBitextMining \cite{singh2024indicgenbench} & 30 (asm, awa, ben, bgc, bho, bod, boy, eng, gbm, gom, guj...) & BitextMining & s2s & Web, News & 1004.5 & 128.5 \\
 \hline 
IndicLangClassification \cite{madhani-etal-2023-bhasa} & 22 (asm, ben, brx, doi, gom, guj, hin, kan, kas, mai, mal...) & Classification & s2s & Web, Non-fiction & 30418.0 & 106.5 \\
 \hline 
IndicNLPNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 8 (guj, kan, mal, mar, ori, pan, tam, tel) & Classification & s2s & News & 2048.0 & 1169.1 \\
 \hline 
IndicQARetrieval \cite{doddapaneni2022towards} & 11 (asm, ben, guj, hin, kan, mal, mar, ory, pan, tam, tel) & Retrieval & s2p & Web & 18586.0 & 930.6 \\
 \hline 
IndicReviewsClusteringP2P \cite{doddapaneni2022towards} & 13 (asm, ben, brx, guj, hin, kan, mal, mar, ory, pan, tam...) & Clustering & p2p & Reviews & 1000.0 & 137.6 \\
 \hline 
IndicSentimentClassification \cite{doddapaneni2022towards} & 13 (asm, ben, brx, guj, hin, kan, mal, mar, ory, pan, tam...) & Classification & s2s & Reviews & 1000.0 & 137.6 \\
 \hline 
IndonesianIdClickbaitClassification \cite{WILLIAM2020106231} & 1 (ind) & Classification & s2s & News & 2048.0 & 64.3 \\
 \hline 
IndonesianMongabayConservationClassification \cite{fransiska-etal-2023-utilizing} & 1 (ind) & Classification & s2s & Web & 977.0 & 1675.7 \\
 \hline 
InsurancePolicyInterpretationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 133.0 & 521.9 \\
 \hline 
InternationalCitizenshipQuestionsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2048.0 & 206.2 \\
 \hline 
IsiZuluNewsClassification \cite{Madodonga_Marivate_Adendorff_2023} & 1 (zul) & Classification & s2s & News & 752.0 & 43.1 \\
 \hline 
ItaCaseholdClassification \cite{10.1145/3594536.3595177} & 1 (ita) & Classification & s2s & Legal, Government & 221.0 & 4207.9 \\
 \hline 
Itacola \cite{trotta-etal-2021-monolingual-cross} & 1 (ita) & Classification & s2s & Non-fiction, Spoken & 4388.0 & 36.3 \\
 \hline 
JCrewBlockerLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 54.0 & 1092.2 \\
 \hline 
JDReview \cite{nielsen-2023-scandeval} & 1 (cmn) & Classification & s2s &  &  &  \\
 \hline 
JSICK \cite{yanaka2022compositional} & 1 (jpn) & STS & s2s & Web & 1986.0 & 21.5 \\
 \hline 
JSTS \cite{kurihara-etal-2022-jglue} & 1 (jpn) & STS & s2s & Web & 1457.0 & 46.3 \\
 \hline 
JaGovFaqsRetrieval  & 1 (jpn) & Retrieval & s2s & Web & 2048.0 & 210.0 \\
 \hline 
JaQuADRetrieval \cite{so2022jaquad} & 1 (jpn) & Retrieval & p2p & Encyclopaedic, Non-fiction & 2048.0 & 400.8 \\
 \hline 
JavaneseIMDBClassification \cite{wongso2021causal} & 1 (jav) & Classification & s2s & Reviews & 25000.0 & 481.8 \\
 \hline 
KLUE-NLI \cite{park2021klue} & 1 (kor) & PairClassification & s2s & News, Encyclopaedic & 2000.0 & 35.0 \\
 \hline 
KLUE-STS \cite{park2021klue} & 1 (kor) & STS & s2s & Reviews, News, Spoken & 519.0 & 33.2 \\
 \hline 
KLUE-TC \cite{park2021klue} & 1 (kor) & Classification & s2s & News & 2048.0 & 27.1 \\
 \hline 
KannadaNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 1 (kan) & Classification & s2s & News & 6460.0 & 65.9 \\
 \hline 
KinopoiskClassification \cite{blinov2013research} & 1 (rus) & Classification & p2p & Reviews & 1500.0 & 1897.3 \\
 \hline 
Ko-StrategyQA \cite{geva2021strategyqa} & 1 (kor) & Retrieval & s2p &  &  &  \\
 \hline 
Ko-miracl \cite{10.1162/tacl_a_00595} & 1 (kor) & Retrieval & s2p &  &  &  \\
 \hline 
KorFin \cite{son2023removing} & 1 (kor) & Classification & s2s & News & 2048.0 & 75.3 \\
 \hline 
KorHateClassification \cite{moon2020beep} & 1 (kor) & Classification & s2s & Social & 1259.5 & 38.7 \\
 \hline 
KorHateSpeechMLClassification \cite{lee-etal-2022-k} & 1 (kor) & MultilabelClassification & s2s & Social & 5120.0 & 34.2 \\
 \hline 
KorSTS \cite{ham2020kornli} & 1 (kor) & STS & s2s & News, Web & 1379.0 & 29.3 \\
 \hline 
KorSarcasmClassification \cite{kim2019kocasm} & 1 (kor) & Classification & s2s & Social & 1174.5 & 47.6 \\
 \hline 
KurdishSentimentClassification \cite{article} & 1 (kur) & Classification & s2s & Web & 3993.5 & 57.7 \\
 \hline 
LCQMC \cite{raghu-etal-2021-end} & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
LEMBNarrativeQARetrieval \cite{kocisky-etal-2018-narrativeqa} & 1 (eng) & Retrieval & s2p & Fiction, Non-fiction & 10804.0 & 326399.3 \\
 \hline 
LEMBNeedleRetrieval \cite{zhu2024longembed} & 1 (eng) & Retrieval & s2p & Academic, Blog & 150.0 & 35305.2 \\
 \hline 
LEMBPasskeyRetrieval \cite{zhu2024longembed} & 1 (eng) & Retrieval & s2p & Fiction & 150.0 & 28994.8 \\
 \hline 
LEMBQMSumRetrieval \cite{zhong-etal-2021-qmsum} & 1 (eng) & Retrieval & s2p & Spoken & 1724.0 & 56136.4 \\
 \hline 
LEMBSummScreenFDRetrieval \cite{chen-etal-2022-summscreen} & 1 (eng) & Retrieval & s2p & Spoken & 672.0 & 31445.8 \\
 \hline 
LEMBWikimQARetrieval \cite{ho2020constructing} & 1 (eng) & Retrieval & s2p & Encyclopaedic & 500.0 & 37513.0 \\
 \hline 
LanguageClassification \cite{conneau2018xnli} & 20 (ara, bul, cmn, deu, ell, eng, fra, hin, ita, jpn, nld...) & Classification & s2s & Reviews, Web, Non-fiction, Fiction, Government & 2048.0 & 107.8 \\
 \hline 
LccSentimentClassification \cite{quasthoff-etal-2006-corpus} & 1 (dan) & Classification & s2s & News, Web & 150.0 & 118.7 \\
 \hline 
LeCaRDv2 \cite{li2023lecardv2} & 1 (zho) & Retrieval & p2p & Legal &  &  \\
 \hline 
LearnedHandsBenefitsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 66.0 & 1308.4 \\
 \hline 
LearnedHandsBusinessLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 174.0 & 1144.5 \\
 \hline 
LearnedHandsConsumerLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 614.0 & 1277.5 \\
 \hline 
LearnedHandsCourtsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 192.0 & 1171.0 \\
 \hline 
LearnedHandsCrimeLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 688.0 & 1212.9 \\
 \hline 
LearnedHandsDivorceLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 150.0 & 1242.4 \\
 \hline 
LearnedHandsDomesticViolenceLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 174.0 & 1360.8 \\
 \hline 
LearnedHandsEducationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 56.0 & 1397.4 \\
 \hline 
LearnedHandsEmploymentLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 710.0 & 1262.7 \\
 \hline 
LearnedHandsEstatesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 178.0 & 1200.7 \\
 \hline 
LearnedHandsFamilyLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2048.0 & 1338.3 \\
 \hline 
LearnedHandsHealthLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 226.0 & 1472.6 \\
 \hline 
LearnedHandsHousingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2048.0 & 1322.5 \\
 \hline 
LearnedHandsImmigrationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 134.0 & 1216.3 \\
 \hline 
LearnedHandsTortsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 432.0 & 1407.0 \\
 \hline 
LearnedHandsTrafficLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 556.0 & 1182.9 \\
 \hline 
LegalBenchConsumerContractsQA \cite{koreeda2021contractnli} & 1 (eng) & Retrieval & s2p & Legal &  &  \\
 \hline 
LegalBenchCorporateLobbying \cite{guha2023legalbench} & 1 (eng) & Retrieval & s2p & Legal &  &  \\
 \hline 
LegalBenchPC \cite{guha2023legalbench} & 1 (eng) & PairClassification & s2s & Legal & 2048.0 & 287.2 \\
 \hline 
LegalQuAD \cite{9723721} & 1 (deu) & Retrieval & s2p & Legal &  &  \\
 \hline 
LegalReasoningCausalityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 55.0 & 1563.8 \\
 \hline 
LegalSummarization \cite{manor-li-2019-plain} & 1 (eng) & Retrieval & s2p & Legal &  &  \\
 \hline 
LivedoorNewsClustering  & 1 (jpn) & Clustering & s2s & News & 1107.0 & 1082.6 \\
 \hline 
MAUDLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2048.0 & 1802.9 \\
 \hline 
MIRACLReranking \cite{10.1162/tacl_a_00595} & 18 (ara, ben, deu, eng, fas, fin, fra, hin, ind, jpn, kor...) & Reranking & s2s & Encyclopaedic & 44608.0 & 506.3 \\
 \hline 
MIRACLRetrieval \cite{10.1162/tacl_a_00595} & 2 (deu, spa) & Retrieval & s2p &  &  &  \\
 \hline 
MLQARetrieval \cite{lewis2019mlqa} & 7 (ara, deu, eng, hin, spa, vie, zho) & Retrieval & s2p & Encyclopaedic & 86915.0 & 37152.5 \\
 \hline 
MLQuestions \cite{kulshreshtha-etal-2021-back} & 1 (eng) & Retrieval & s2p & Encyclopaedic, Academic & 1500.0 & 306.0 \\
 \hline 
MLSUMClusteringP2P.v2 \cite{scialom2020mlsum} & 4 (deu, fra, rus, spa) & Clustering & p2p & News & 2048.0 & 4711.5 \\
 \hline 
MLSUMClusteringS2S.v2 \cite{scialom2020mlsum} & 4 (deu, fra, rus, spa) & Clustering & s2s & News & 2048.0 & 4711.5 \\
 \hline 
MMarcoReranking \cite{bonifacio2021mmarco} & 1 (cmn) & Reranking & s2s &  &  &  \\
 \hline 
MMarcoRetrieval \cite{xiao2024cpack} & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
MSMARCO \cite{DBLP:journals/corr/NguyenRSGTMD16} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
MSMARCO-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
MSMARCOv2 \cite{DBLP:journals/corr/NguyenRSGTMD16} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
MTOPDomainClassification \cite{li-etal-2021-mtop} & 6 (deu, eng, fra, hin, spa, tha) & Classification & s2s & Spoken & 3310.5 & 36.6 \\
 \hline 
MTOPIntentClassification \cite{li-etal-2021-mtop} & 6 (deu, eng, fra, hin, spa, tha) & Classification & s2s & Spoken & 3310.5 & 36.6 \\
 \hline 
MacedonianTweetSentimentClassification \cite{jovanoski-etal-2015-sentiment} & 1 (mkd) & Classification & s2s & Social & 1139.0 & 67.6 \\
 \hline 
MalayalamNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 1 (mal) & Classification & s2s & News & 3148.0 & 80.0 \\
 \hline 
MalteseNewsClassification \cite{maltese-news-datasets} & 1 (mlt) & MultilabelClassification & s2s & Constructed & 6540.5 & 1673.9 \\
 \hline 
MarathiNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 1 (mar) & Classification & s2s & News & 2048.0 & 52.4 \\
 \hline 
MasakhaNEWSClassification \cite{adelani2023masakhanews} & 16 (amh, eng, fra, hau, ibo, lin, lug, orm, pcm, run, sna...) & Classification & s2s & News & 422.0 & 5116.6 \\
 \hline 
MasakhaNEWSClusteringP2P \cite{Adelani2023MasakhaNEWS} & 16 (amh, eng, fra, hau, ibo, lin, lug, orm, pcm, run, sna...) & Clustering & p2p &  &  &  \\
 \hline 
MasakhaNEWSClusteringS2S \cite{Adelani2023MasakhaNEWS} & 16 (amh, eng, fra, hau, ibo, lin, lug, orm, pcm, run, sna...) & Clustering & s2s &  &  &  \\
 \hline 
MassiveIntentClassification \cite{fitzgerald2022massive} & 50 (afr, amh, ara, aze, ben, cmo, cym, dan, deu, ell, eng...) & Classification & s2s & Spoken & 2503.5 & 34.7 \\
 \hline 
MassiveScenarioClassification \cite{fitzgerald2022massive} & 50 (afr, amh, ara, aze, ben, cmo, cym, dan, deu, ell, eng...) & Classification & s2s & Spoken & 2503.5 & 34.7 \\
 \hline 
MedicalQARetrieval \cite{BenAbacha-BMC-2019} & 1 (eng) & Retrieval & s2s & Medical & 2048.0 & 1206.0 \\
 \hline 
MedicalRetrieval  & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
MedrxivClusteringP2P.v2  & 1 (eng) & Clustering & p2p & Academic, Medical & 2048.0 & 1984.7 \\
 \hline 
MedrxivClusteringS2S.v2  & 1 (eng) & Clustering & s2s & Academic, Medical & 2048.0 & 114.9 \\
 \hline 
MewsC16JaClustering \cite{nishikawa-etal-2022-ease} & 1 (jpn) & Clustering & s2s & News & 992.0 & 95.0 \\
 \hline 
MindSmallReranking \cite{wu-etal-2020-mind} & 1 (eng) & Reranking & s2s & News & 107968.0 & 70.9 \\
 \hline 
MintakaRetrieval \cite{sen-etal-2022-mintaka} & 8 (ara, deu, fra, hin, ita, jpn, por, spa) & Retrieval & s2p &  &  &  \\
 \hline 
Moroco \cite{Butnaru-ACL-2019} & 1 (ron) & Classification & s2s & News & 2048.0 & 1710.9 \\
 \hline 
MovieReviewSentimentClassification \cite{blard2020} & 1 (fra) & Classification & s2s & Reviews & 1024.0 & 554.2 \\
 \hline 
MultiEURLEXMultilabelClassification \cite{chalkidis-etal-2021-multieurlex} & 23 (bul, ces, dan, deu, ell, eng, est, fin, fra, hrv, hun...) & MultilabelClassification & p2p & Legal, Government & 5000.0 & 12014.4 \\
 \hline 
MultiHateClassification \cite{rottger-etal-2021-hatecheck} & 11 (ara, cmn, deu, eng, fra, hin, ita, nld, pol, por, spa) & Classification & s2s & Constructed & 10000.0 & 45.9 \\
 \hline 
MultiLongDocRetrieval \cite{bge-m3} & 13 (ara, cmn, deu, eng, fra, hin, ita, jpn, kor, por, rus...) & Retrieval & s2p &  &  &  \\
 \hline 
MultilingualSentiment  & 1 (cmn) & Classification & s2s &  &  &  \\
 \hline 
MultilingualSentimentClassification \cite{mollanorozy-etal-2023-cross} & 29 (ara, bam, bul, cmn, cym, deu, dza, ell, eng, eus, fas...) & Classification & s2s & Reviews & 7000.0 & 56.0 \\
 \hline 
MyanmarNews \cite{Khine2017} & 1 (mya) & Classification & p2p & News & 2048.0 & 174.2 \\
 \hline 
NFCorpus \cite{boteva2016} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
NFCorpus-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
NLPJournalAbsIntroRetrieval  & 1 (jpn) & Retrieval & s2s & Academic & 404.0 & 1246.5 \\
 \hline 
NLPJournalTitleAbsRetrieval  & 1 (jpn) & Retrieval & s2s & Academic & 404.0 & 234.6 \\
 \hline 
NLPJournalTitleIntroRetrieval  & 1 (jpn) & Retrieval & s2s & Academic & 404.0 & 1040.2 \\
 \hline 
NQ \cite{47761} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
NQ-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
NTREXBitextMining \cite{federmann-etal-2022-ntrex} & 119 (afr, amh, arb, aze, bak, bel, bem, ben, bod, bos, bul...) & BitextMining & s2s & News & 3826252.0 & 120.0 \\
 \hline 
NYSJudicialEthicsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 292.0 & 159.4 \\
 \hline 
NaijaSenti \cite{muhammad-etal-2022-naijasenti} & 4 (hau, ibo, pcm, yor) & Classification & s2s & Social & 4800.0 & 72.8 \\
 \hline 
NarrativeQARetrieval \cite{kočiský2017narrativeqa} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
NepaliNewsClassification \cite{arora-2020-inltk} & 1 (nep) & Classification & s2s & News & 3735.0 & 196.3 \\
 \hline 
NeuCLIR2022Retrieval \cite{lawrie2023overview} & 3 (fas, rus, zho) & Retrieval & s2p & News & 3346370.0 & 3086.1 \\
 \hline 
NeuCLIR2023Retrieval \cite{lawrie2024overview} & 3 (fas, rus, zho) & Retrieval & s2p & News & 3346332.0 & 3250.3 \\
 \hline 
News21InstructionRetrieval \cite{weller2024followir} & 1 (eng) & InstructionRetrieval & s2p & News & 61906.0 & 2983.7 \\
 \hline 
NewsClassification \cite{NIPS2015_250cf8b5} & 1 (eng) & Classification & s2s & News & 7600.0 & 235.3 \\
 \hline 
NoRecClassification \cite{velldal-etal-2018-norec} & 1 (nob) & Classification & s2s &  & 2050.0 & 82.0 \\
 \hline 
NollySentiBitextMining \cite{shode2023nollysenti} & 5 (eng, hau, ibo, pcm, yor) & BitextMining & s2s & Social, Reviews & 1640.0 & 135.9 \\
 \hline 
NorQuadRetrieval \cite{ivanova-etal-2023-norquad} & 1 (nob) & Retrieval & p2p & Encyclopaedic, Non-fiction & 2602.0 & 502.2 \\
 \hline 
NordicLangClassification \cite{haas-derczynski-2021-discriminating} & 6 (dan, fao, isl, nno, nob, swe) & Classification & s2s &  & 3000.0 & 78.2 \\
 \hline 
NorwegianCourtsBitextMining \cite{opus4} & 2 (nno, nob) & BitextMining & s2s & Legal & 2050.0 & 1884.0 \\
 \hline 
NorwegianParliamentClassification \cite{kummervold-etal-2021-operationalizing} & 1 (nob) & Classification & s2s &  & 1200.0 & 1897.5 \\
 \hline 
NusaParagraphEmotionClassification \cite{cahyawijaya-etal-2023-nusawrites} & 10 (bbc, bew, bug, jav, mad, mak, min, mui, rej, sun) & Classification & s2s & Non-fiction, Fiction & 8238.0 & 740.5 \\
 \hline 
NusaParagraphTopicClassification \cite{cahyawijaya-etal-2023-nusawrites} & 10 (bbc, bew, bug, jav, mad, mak, min, mui, rej, sun) & Classification & s2s & Non-fiction, Fiction & 8238.0 & 740.5 \\
 \hline 
NusaTranslationBitextMining \cite{cahyawijaya2023nusawrites} & 12 (abs, bbc, bew, bhp, ind, jav, mad, mak, min, mui, rej...) & BitextMining & s2s & Social & 50200.0 & 147.0 \\
 \hline 
NusaX-senti \cite{winata2022nusax} & 12 (ace, ban, bbc, bjn, bug, eng, ind, jav, mad, min, nij...) & Classification & s2s & Reviews, Web, Social, Constructed & 4800.0 & 52.4 \\
 \hline 
NusaXBitextMining \cite{winata2023nusax} & 12 (ace, ban, bbc, bjn, bug, eng, ind, jav, mad, min, nij...) & BitextMining & s2s & Reviews & 5500.0 & 157.2 \\
 \hline 
OPP115DataRetentionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 88.0 & 195.2 \\
 \hline 
OPP115DataSecurityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1334.0 & 246.7 \\
 \hline 
OPP115DoNotTrackLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 110.0 & 223.2 \\
 \hline 
OPP115FirstPartyCollectionUseLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2086.0 & 204.2 \\
 \hline 
OPP115InternationalAndSpecificAudiencesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 980.0 & 327.7 \\
 \hline 
OPP115PolicyChangeLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 431.0 & 201.0 \\
 \hline 
OPP115ThirdPartySharingCollectionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1590.0 & 223.6 \\
 \hline 
OPP115UserAccessEditAndDeletionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 462.0 & 218.6 \\
 \hline 
OPP115UserChoiceControlLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 1546.0 & 210.6 \\
 \hline 
Ocnli \cite{hu2020ocnli} & 1 (cmn) & PairClassification & s2s &  &  &  \\
 \hline 
OdiaNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 1 (ory) & Classification & s2s & News & 2048.0 & 49.2 \\
 \hline 
OnlineShopping \cite{nielsen-2023-scandeval} & 1 (cmn) & Classification & s2s &  &  &  \\
 \hline 
OnlineStoreReviewSentimentClassification  & 1 (ara) & Classification & s2s & Reviews & 2048.0 & 137.2 \\
 \hline 
OpusparcusPC \cite{creutz2018open} & 6 (deu, eng, fin, fra, rus, swe) & PairClassification & s2s &  &  &  \\
 \hline 
OralArgumentQuestionPurposeLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 312.0 & 269.7 \\
 \hline 
OverrulingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2048.0 & 167.2 \\
 \hline 
PAC  & 1 (pol) & Classification & p2p &  & 3453.0 & 185.3 \\
 \hline 
PAWSX \cite{raghu-etal-2021-end} & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
PIQA \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 1838.0 & 134.3 \\
 \hline 
PROALegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 95.0 & 251.7 \\
 \hline 
PSC \cite{ogrodniczuk-kopec-2014-polish} & 1 (pol) & PairClassification & s2s &  &  &  \\
 \hline 
PatentClassification \cite{sharma-etal-2019-bigpatent} & 1 (eng) & Classification & s2s & Legal & 5000.0 & 18620.4 \\
 \hline 
PawsX \cite{yang2019pawsx} & 7 (cmn, deu, eng, fra, jpn, kor, spa) & PairClassification & s2s &  &  &  \\
 \hline 
PersianFoodSentimentClassification \cite{ParsBERT} & 1 (fas) & Classification & s2s & Reviews & 2048.0 & 90.5 \\
 \hline 
PersonalJurisdictionLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 50.0 & 381.1 \\
 \hline 
PlscClusteringP2P.v2  & 1 (pol) & Clustering & s2s & Academic & 2048.0 & 1023.2 \\
 \hline 
PlscClusteringS2S.v2  & 1 (pol) & Clustering & s2s & Academic & 2048.0 & 84.3 \\
 \hline 
PoemSentimentClassification \cite{sheng2020investigating} & 1 (eng) & Classification & s2s & Reviews & 104.5 & 43.8 \\
 \hline 
PolEmo2.0-IN \cite{kocon-etal-2019-multi} & 1 (pol) & Classification & s2s &  &  &  \\
 \hline 
PolEmo2.0-OUT  & 1 (pol) & Classification & s2s &  & 722.0 & 756.2 \\
 \hline 
PpcPC \cite{dadas2022training} & 1 (pol) & PairClassification & s2s &  &  &  \\
 \hline 
PublicHealthQA \cite{xing_han_lu_2024} & 8 (ara, eng, fra, kor, rus, spa, vie, zho) & Retrieval & s2p & Medical, Government, Web & 888.0 & 778.2 \\
 \hline 
PunjabiNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 1 (pan) & Classification & s2s & News & 392.0 & 4168.7 \\
 \hline 
QBQTC  & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
Quail \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 2720.0 & 1983.3 \\
 \hline 
Quora-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2s &  &  &  \\
 \hline 
QuoraRetrieval \cite{quora-question-pairs} & 1 (eng) & Retrieval & s2s &  &  &  \\
 \hline 
RARbCode \cite{xiao2024rar} & 1 (eng) & Retrieval & s2p & Programming & 1484.0 & 621.2 \\
 \hline 
RARbMath \cite{xiao2024rar} & 1 (eng) & Retrieval & s2p & Encyclopaedic & 6319.0 & 682.9 \\
 \hline 
RTE3 \cite{giampiccolo-etal-2007-third} & 4 (deu, eng, fra, ita) & PairClassification & s2s & News, Web, Encyclopaedic & 1923.0 & 124.8 \\
 \hline 
RUParaPhraserSTS \cite{gudkov-etal-2020-automatically} & 1 (rus) & STS & s2s & News & 1924.0 & 61.2 \\
 \hline 
RedditClusteringP2P.v2 \cite{geigle:2021:arxiv} & 1 (eng) & Clustering & p2p & Web, Social & 16000.0 & 727.7 \\
 \hline 
RedditClusteringS2S.v2 \cite{geigle:2021:arxiv} & 1 (eng) & Clustering & s2s & Web, Social & 16000.0 & 64.7 \\
 \hline 
RestaurantReviewSentimentClassification \cite{elsahar2015building} & 1 (ara) & Classification & s2s & Reviews & 2048.0 & 231.4 \\
 \hline 
RiaNewsRetrieval \cite{gavrilov2018self} & 1 (rus) & Retrieval & s2p & News & 10000.0 & 1230.8 \\
 \hline 
Robust04InstructionRetrieval \cite{weller2024followir} & 1 (eng) & InstructionRetrieval & s2p & News & 95088.0 & 2471.0 \\
 \hline 
RomaTalesBitextMining  & 2 (hun, rom) & BitextMining & s2s & Fiction & 215.0 & 316.8 \\
 \hline 
RomaniBibleClustering  & 1 (rom) & Clustering & p2p & Religious & 2048.0 & 132.2 \\
 \hline 
RomanianReviewsSentiment \cite{tache2101clustering} & 1 (ron) & Classification & s2s & Reviews & 2048.0 & 588.6 \\
 \hline 
RomanianSentimentClassification \cite{dumitrescu2020birth} & 1 (ron) & Classification & s2s & Reviews & 2048.0 & 67.6 \\
 \hline 
RonSTS \cite{dumitrescu2021liro} & 1 (ron) & STS & s2s & News, Social, Web & 1379.0 & 60.5 \\
 \hline 
RuBQReranking \cite{RuBQ2021} & 1 (rus) & Reranking & s2p & Encyclopaedic & 1551.0 & 499.9 \\
 \hline 
RuBQRetrieval \cite{RuBQ2021} & 1 (rus) & Retrieval & s2p & Encyclopaedic & 2845.0 & 509.5 \\
 \hline 
RuReviewsClassification \cite{Smetanin-SA-2019} & 1 (rus) & Classification & p2p & Reviews & 2048.0 & 133.2 \\
 \hline 
RuSTSBenchmarkSTS \cite{huggingface:dataset:stsb_multi_mt} & 1 (rus) & STS & s2s & News, Social, Web & 1264.0 & 54.2 \\
 \hline 
RuSciBenchGRNTIClassification  & 1 (rus) & Classification & p2p & Academic & 2048.0 & 890.1 \\
 \hline 
RuSciBenchGRNTIClusteringP2P  & 1 (rus) & Clustering & p2p & Academic & 2048.0 & 890.1 \\
 \hline 
RuSciBenchOECDClassification  & 1 (rus) & Classification & p2p & Academic & 2048.0 & 838.9 \\
 \hline 
RuSciBenchOECDClusteringP2P  & 1 (rus) & Clustering & p2p & Academic & 2048.0 & 838.9 \\
 \hline 
SCDBPAccountabilityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3520.0 \\
 \hline 
SCDBPAuditsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3507.0 \\
 \hline 
SCDBPCertificationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 378.0 & 3507.0 \\
 \hline 
SCDBPTrainingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3506.0 \\
 \hline 
SCDBPVerificationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3498.0 \\
 \hline 
SCDDAccountabilityLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 378.0 & 3522.0 \\
 \hline 
SCDDAuditsLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3506.0 \\
 \hline 
SCDDCertificationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 378.0 & 3518.0 \\
 \hline 
SCDDTrainingLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3499.0 \\
 \hline 
SCDDVerificationLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 379.0 & 3503.0 \\
 \hline 
SCIDOCS \cite{specter2020cohan} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
SCIDOCS-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
SIB200Classification \cite{adelani2023sib} & 197 (ace, acm, acq, aeb, afr, ajp, aka, als, amh, apc, arb...) & Classification & s2s & News & 334.7 & 114.6 \\
 \hline 
SIB200ClusteringS2S \cite{adelani2023sib} & 197 (ace, acm, acq, aeb, afr, ajp, aka, als, amh, apc, arb...) & Clustering & s2s & News & 1004.0 & 114.8 \\
 \hline 
SICK-BR-PC \cite{real18} & 1 (por) & PairClassification & s2s & Web & 1000.0 & 54.9 \\
 \hline 
SICK-BR-STS \cite{real18} & 1 (por) & STS & s2s & Web & 1000.0 & 54.9 \\
 \hline 
SICK-E-PL \cite{dadas-etal-2020-evaluation} & 1 (pol) & PairClassification & s2s &  &  &  \\
 \hline 
SICK-R \cite{marelli-etal-2014-sick} & 1 (eng) & STS & s2s &  &  &  \\
 \hline 
SICK-R-PL \cite{dadas-etal-2020-evaluation} & 1 (pol) & STS & s2s & Web & 9812.0 & 42.8 \\
 \hline 
SICKFr  & 1 (fra) & STS & s2s &  &  &  \\
 \hline 
SIQA \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 0.0 & 0.0 \\
 \hline 
SNLHierarchicalClusteringP2P \cite{navjord2023beyond} & 1 (nob) & Clustering & p2p & Encyclopaedic, Non-fiction & 1300.0 & 1986.9 \\
 \hline 
SNLHierarchicalClusteringS2S \cite{navjord2023beyond} & 1 (nob) & Clustering & s2s & Encyclopaedic, Non-fiction & 1300.0 & 242.2 \\
 \hline 
SNLRetrieval \cite{navjord2023beyond} & 1 (nob) & Retrieval & p2p & Encyclopaedic, Non-fiction & 2048.0 & 1101.3 \\
 \hline 
SRNCorpusBitextMining \cite{zwennicker2022towards} & 2 (nld, srn) & BitextMining & s2s & Social, Web & 256.0 & 55.0 \\
 \hline 
STS12 \cite{10.5555/2387636.2387697} & 1 (eng) & STS & s2s & Encyclopaedic, News & 6216.0 & 64.7 \\
 \hline 
STS13 \cite{Agirre2013SEM2S} & 1 (eng) & STS & s2s & Web, News, Non-fiction & 3000.0 & 54.0 \\
 \hline 
STS14 \cite{bandhakavi-etal-2014-generating} & 1 (eng) & STS & s2s & Blog, Web & 7500.0 & 54.3 \\
 \hline 
STS15 \cite{bicici-2015-rtm} & 1 (eng) & STS & s2s & Blog, News, Web & 6000.0 & 57.7 \\
 \hline 
STS16 \cite{nakov-etal-2016-semeval} & 1 (eng) & STS & s2s & Blog, Web & 2372.0 & 65.3 \\
 \hline 
STS17 \cite{cer-etal-2017-semeval} & 9 (ara, deu, eng, fra, ita, kor, nld, spa, tur) & STS & s2s & News, Web & 500.0 & 43.3 \\
 \hline 
STS22 \cite{chen-etal-2022-semeval} & 10 (ara, cmn, deu, eng, fra, ita, pol, rus, spa, tur) & STS & p2p & News & 8056.0 & 1993.6 \\
 \hline 
STSB \cite{raghu-etal-2021-end} & 1 (cmn) & STS & s2s &  &  &  \\
 \hline 
STSBenchmark \cite{huggingface:dataset:stsb_multi_mt} & 1 (eng) & STS & s2s &  &  &  \\
 \hline 
STSBenchmarkMultilingualSTS \cite{huggingface:dataset:stsb_multi_mt} & 10 (cmn, deu, eng, fra, ita, nld, pol, por, rus, spa) & STS & s2s & News, Social, Web & 28790.0 & 61.3 \\
 \hline 
STSES \cite{agirre2015semeval} & 1 (spa) & STS & s2s &  &  &  \\
 \hline 
SanskritShlokasClassification \cite{arora-2020-inltk} & 1 (san) & Classification & s2s & Religious & 239.5 & 97.5 \\
 \hline 
ScalaClassification \cite{nielsen-2023-scandeval} & 4 (dan, nno, nob, swe) & Classification & s2s & Fiction, News, Non-fiction, Blog, Spoken, Web & 4096.0 & 102.7 \\
 \hline 
SciDocsRR \cite{cohan-etal-2020-specter} & 1 (eng) & Reranking & s2s & Academic, Non-fiction & 19599.0 & 69.0 \\
 \hline 
SciFact \cite{specter2020cohan} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
SciFact-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
SemRel24STS \cite{ousidhoum2024semrel2024} & 12 (afr, amh, arb, arq, ary, eng, hau, hin, ind, kin, mar...) & STS & s2s &  & 4793.5 & 154.5 \\
 \hline 
SensitiveTopicsClassification \cite{babakov-etal-2021-detecting} & 1 (rus) & MultilabelClassification & s2s & Web, Social & 2048.0 & 95.3 \\
 \hline 
SentimentAnalysisHindi \cite{OdiaGenAI} & 1 (hin) & Classification & s2s & Reviews & 2497.0 & 81.3 \\
 \hline 
SinhalaNewsClassification \cite{deSilva2015} & 1 (sin) & Classification & s2s & News & 3327.0 & 148.0 \\
 \hline 
SinhalaNewsSourceClassification \cite{dhananjaya2022} & 1 (sin) & Classification & s2s & News & 24094.0 & 56.1 \\
 \hline 
SiswatiNewsClassification \cite{Madodonga_Marivate_Adendorff_2023} & 1 (ssw) & Classification & s2s & News & 80.0 & 354.2 \\
 \hline 
SlovakMovieReviewSentimentClassification \cite{vstefanik2023resources} & 1 (svk) & Classification & s2s & Reviews & 2048.0 & 366.2 \\
 \hline 
SlovakSumRetrieval \cite{OndrejowaSlovakSum24} & 1 (slk) & Retrieval & s2s & News, Social, Web & 600.0 & 238.4 \\
 \hline 
SouthAfricanLangClassification \cite{south-african-language-identification} & 11 (afr, eng, nbl, nso, sot, ssw, tsn, tso, ven, xho, zul) & Classification & s2s & Web, Non-fiction & 2048.0 & 247.5 \\
 \hline 
SpanishNewsClassification  & 1 (spa) & Classification & s2s & News & 2048.0 & 4218.2 \\
 \hline 
SpanishNewsClusteringP2P  & 1 (spa) & Clustering & p2p &  &  &  \\
 \hline 
SpanishPassageRetrievalS2P \cite{10.1007/978-3-030-15719-7_19} & 1 (spa) & Retrieval & s2p &  &  &  \\
 \hline 
SpanishPassageRetrievalS2S \cite{10.1007/978-3-030-15719-7_19} & 1 (spa) & Retrieval & s2s &  &  &  \\
 \hline 
SpanishSentimentClassification \cite{mollanorozy-etal-2023-cross} & 1 (spa) & Classification & s2s & Reviews & 221.5 & 86.5 \\
 \hline 
SpartQA \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 0.0 & 0.0 \\
 \hline 
SprintDuplicateQuestions \cite{shah-etal-2018-adversarial} & 1 (eng) & PairClassification & s2s &  & 101000.0 & 66.6 \\
 \hline 
StackExchangeClustering.v2 \cite{geigle:2021:arxiv} & 1 (eng) & Clustering & s2s & Web & 16000.0 & 57.0 \\
 \hline 
StackExchangeClusteringP2P.v2 \cite{geigle:2021:arxiv} & 1 (eng) & Clustering & p2p & Web & 16000.0 & 1090.7 \\
 \hline 
StackOverflowDupQuestions \cite{Liu2018LinkSOAD} & 1 (eng) & Reranking & s2s &  & 3467.0 & 49.8 \\
 \hline 
StatcanDialogueDatasetRetrieval \cite{lu-etal-2023-statcan} & 2 (eng, fra) & Retrieval & s2p & Government, Web & 2639.3 & 2813.6 \\
 \hline 
SummEval \cite{10.1093/bioinformatics/btx238} & 1 (eng) & Summarization & p2p &  & 2800.0 & 359.8 \\
 \hline 
SummEvalFr \cite{fabbri2020summeval} & 1 (fra) & Summarization & p2p &  &  &  \\
 \hline 
SweFaqRetrieval  & 1 (swe) & Retrieval & s2s & Government, Non-fiction & 1024.0 & 195.4 \\
 \hline 
SweRecClassification \cite{nielsen-2023-scandeval} & 1 (swe) & Classification & s2s &  & 1024.0 & 318.8 \\
 \hline 
SwedishSentimentClassification  & 1 (swe) & Classification & s2s & Reviews & 1024.0 & 498.7 \\
 \hline 
SwednClusteringP2P \cite{monsen2021method} & 1 (swe) & Clustering & p2p & News, Non-fiction & 2048.0 & 1619.7 \\
 \hline 
SwednClusteringS2S \cite{monsen2021method} & 1 (swe) & Clustering & s2s & News, Non-fiction & 2048.0 & 1619.7 \\
 \hline 
SwednRetrieval \cite{monsen2021method} & 1 (swe) & Retrieval & p2p & News, Non-fiction & 2048.0 & 1946.3 \\
 \hline 
SwissJudgementClassification \cite{niklaus2022empirical} & 3 (deu, fra, ita) & Classification & s2s & Legal & 2048.0 & 3411.7 \\
 \hline 
SyntecReranking \cite{ciancone2024extending} & 1 (fra) & Reranking & s2p & Legal &  &  \\
 \hline 
SyntecRetrieval \cite{ciancone2024extending} & 1 (fra) & Retrieval & s2p & Legal & 90.0 & 62.0 \\
 \hline 
T2Reranking \cite{xie2023t2ranking} & 1 (cmn) & Reranking & s2s &  &  &  \\
 \hline 
T2Retrieval \cite{xie2023t2ranking} & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
TERRa \cite{shavrina2020russiansuperglue} & 1 (rus) & PairClassification & s2s & News, Web & 307.0 & 138.2 \\
 \hline 
TNews \cite{xu-etal-2020-clue} & 1 (cmn) & Classification & s2s &  &  &  \\
 \hline 
TRECCOVID \cite{roberts2021searching} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
TRECCOVID-PL \cite{wojtasik2024beirpl} & 1 (pol) & Retrieval & s2p &  &  &  \\
 \hline 
TV2Nordretrieval \cite{flansmose-mikkelsen-etal-2022-ddisco} & 1 (dan) & Retrieval & p2p & News, Non-fiction & 4096.0 & 784.1 \\
 \hline 
TamilNewsClassification \cite{kunchukuttan2020indicnlpcorpus} & 1 (tam) & Classification & s2s & News & 9076.0 & 56.5 \\
 \hline 
Tatoeba \cite{tatoeba} & 113 (afr, amh, ang, ara, arq, arz, ast, awa, aze, bel, ben...) & BitextMining & s2s &  & 2000.0 & 39.4 \\
 \hline 
TbilisiCityHallBitextMining  & 2 (eng, kat) & BitextMining & s2s & News & 1820.0 & 78.0 \\
 \hline 
TelemarketingSalesRuleLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 47.0 & 348.3 \\
 \hline 
TeluguAndhraJyotiNewsClassification  & 1 (tel) & Classification & s2s & News & 4329.0 & 1428.3 \\
 \hline 
TempReasonL1 \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 4000.0 & 59.2 \\
 \hline 
TempReasonL2Context \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 0.0 & 0.0 \\
 \hline 
TempReasonL2Fact \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 5397.0 & 854.8 \\
 \hline 
TempReasonL2Pure \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 5397.0 & 80.0 \\
 \hline 
TempReasonL3Context \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 4426.0 & 13448.4 \\
 \hline 
TempReasonL3Fact \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 4426.0 & 919.9 \\
 \hline 
TempReasonL3Pure \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 4426.0 & 98.2 \\
 \hline 
TenKGnadClassification \cite{Schabus2017} & 1 (deu) & Classification & p2p & News & 1028.0 & 2627.3 \\
 \hline 
TenKGnadClusteringP2P.v2  & 1 (deu) & Clustering & p2p & News, Non-fiction & 10275.0 & 2641.0 \\
 \hline 
TenKGnadClusteringS2S.v2  & 1 (deu) & Clustering & s2s & News, Non-fiction & 10275.0 & 51.0 \\
 \hline 
TextualismToolDictionariesLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 107.0 & 943.2 \\
 \hline 
TextualismToolPlainLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 165.0 & 998.0 \\
 \hline 
ThuNewsClusteringP2P.v2 \cite{THUCTC} & 1 (cmn) & Clustering & p2p & News & 2048.0 &  \\
 \hline 
ThuNewsClusteringS2S.v2 \cite{THUCTC} & 1 (cmn) & Clustering & s2s & News & 2048.0 &  \\
 \hline 
TopiOCQA \cite{adlakha2022topiocqa} & 1 (eng) & Retrieval & s2p & Encyclopaedic & 2514.0 & 708.0 \\
 \hline 
Touche2020 \cite{potthast_2022_6862281} & 1 (eng) & Retrieval & s2p &  &  &  \\
 \hline 
ToxicChatClassification \cite{lin2023toxicchat} & 1 (eng) & Classification & s2s & Constructed & 1427.0 & 189.4 \\
 \hline 
ToxicConversationsClassification \cite{jigsaw-unintended-bias-in-toxicity-classification} & 1 (eng) & Classification & s2s & Social & 50000.0 & 296.6 \\
 \hline 
TswanaNewsClassification \cite{marivate2023puoberta} & 1 (tsn) & Classification & s2s & News & 487.0 & 2393.6 \\
 \hline 
TurHistQuadRetrieval \cite{9559013} & 1 (tur) & Retrieval & p2p & Encyclopaedic, Non-fiction, Academic & 1330.0 & 1513.8 \\
 \hline 
TurkicClassification  & 3 (bak, kaz, kir) & Classification & s2s & News & 193056.0 & 1103.1 \\
 \hline 
TurkishMovieSentimentClassification \cite{Demirtas2013CrosslingualPD} & 1 (tur) & Classification & s2s & Reviews & 2644.0 & 141.5 \\
 \hline 
TurkishProductSentimentClassification \cite{Demirtas2013CrosslingualPD} & 1 (tur) & Classification & s2s & Reviews & 800.0 & 246.8 \\
 \hline 
TweetEmotionClassification \cite{al2018emotional} & 1 (ara) & Classification & s2s & Social & 2048.0 & 78.8 \\
 \hline 
TweetSarcasmClassification \cite{abu-farha-magdy-2020-arabic} & 1 (ara) & Classification & s2s & Social & 2110.0 & 102.1 \\
 \hline 
TweetSentimentClassification \cite{barbieri-etal-2022-xlm} & 8 (ara, deu, eng, fra, hin, ita, por, spa) & Classification & s2s & Social & 2048.0 & 83.5 \\
 \hline 
TweetSentimentExtractionClassification \cite{tweet-sentiment-extraction} & 1 (eng) & Classification & s2s & Social & 3534.0 & 67.8 \\
 \hline 
TweetTopicSingleClassification \cite{dimosthenis-etal-2022-twitter} & 1 (eng) & Classification & s2s & Social, News & 1693.0 & 167.7 \\
 \hline 
TwentyNewsgroupsClustering.v2 \cite{LANG1995331} & 1 (eng) & Clustering & s2s & News & 2048.0 & 32.0 \\
 \hline 
TwitterHjerneRetrieval \cite{holm2024gllms} & 1 (dan) & Retrieval & p2p & Social & 340.0 & 138.2 \\
 \hline 
TwitterSemEval2015 \cite{xu-etal-2015-semeval} & 1 (eng) & PairClassification & s2s &  & 16777.0 & 38.3 \\
 \hline 
TwitterURLCorpus \cite{lan-etal-2017-continuously} & 1 (eng) & PairClassification & s2s &  & 51534.0 & 79.5 \\
 \hline 
UCCVCommonLawLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 94.0 & 114.1 \\
 \hline 
UkrFormalityClassification \cite{rao-tetreault-2018-dear} & 1 (ukr) & Classification & s2s & News & 2048.0 & 52.6 \\
 \hline 
UnfairTOSLegalBenchClassification \cite{guha2023legalbench} & 1 (eng) & Classification & s2s & Legal & 2048.0 & 184.7 \\
 \hline 
UrduRomanSentimentClassification \cite{misc_roman_urdu_data_set_458} & 1 (urd) & Classification & s2s & Social & 2048.0 & 68.2 \\
 \hline 
VGHierarchicalClusteringP2P \cite{navjord2023beyond} & 1 (nob) & Clustering & p2p & News, Non-fiction & 2048.0 & 2670.3 \\
 \hline 
VGHierarchicalClusteringS2S \cite{navjord2023beyond} & 1 (nob) & Clustering & p2p & News, Non-fiction & 2048.0 & 139.3 \\
 \hline 
VideoRetrieval  & 1 (cmn) & Retrieval & s2p &  &  &  \\
 \hline 
VieMedEVBitextMining \cite{medev} & 2 (eng, vie) & BitextMining & s2s & Medical & 2048.0 & 139.2 \\
 \hline 
VieQuADRetrieval \cite{nguyen-etal-2020-vietnamese} & 1 (vie) & Retrieval & s2p & Encyclopaedic, Non-fiction & 2048.0 & 790.2 \\
 \hline 
VieStudentFeedbackClassification \cite{8573337} & 1 (vie) & Classification & s2s & Reviews & 2048.0 & 14.2 \\
 \hline 
WRIMEClassification \cite{kajiwara-etal-2021-wrime} & 1 (jpn) & Classification & s2s & Social & 2048.0 & 47.8 \\
 \hline 
Waimai \cite{nielsen-2023-scandeval} & 1 (cmn) & Classification & s2s &  &  &  \\
 \hline 
WebLINXCandidatesReranking \cite{lù2024weblinx} & 1 (eng) & Reranking & p2p & Academic, Web & 3276.2 & 1805.2 \\
 \hline 
WikiCitiesClustering \cite{wikidump} & 1 (eng) & Clustering & p2p &  &  &  \\
 \hline 
WikiClusteringP2P.v2  & 14 (bos, cat, ces, dan, eus, glv, ilo, kur, lav, min, mlt...) & Clustering & p2p & Encyclopaedic & 2048.0 & 625.3 \\
 \hline 
WikipediaRerankingMultilingual \cite{wikidump} & 16 (ben, bul, ces, dan, deu, eng, fas, fin, hin, ita, nld...) & Reranking & s2p & Encyclopaedic & 1500.0 & 452.0 \\
 \hline 
WikipediaRetrievalMultilingual  & 16 (ben, bul, ces, dan, deu, eng, fas, fin, hin, ita, nld...) & Retrieval & s2p & Encyclopaedic & 1500.0 & 452.0 \\
 \hline 
WinoGrande \cite{xiao2024rar} & 1 (eng) & Retrieval & s2s & Encyclopaedic & 0.0 & 0.0 \\
 \hline 
WisesightSentimentClassification \cite{bact_2019_3457447} & 1 (tha) & Classification & s2s & Social, News & 2048.0 & 103.4 \\
 \hline 
XMarket \cite{Bonab_2021} & 3 (deu, eng, spa) & Retrieval & s2p &  &  &  \\
 \hline 
XNLI \cite{conneau2018xnli} & 14 (ara, bul, deu, ell, eng, fra, hin, rus, spa, swa, tha...) & PairClassification & s2s & Non-fiction, Fiction, Government & 2311.5 & 106.5 \\
 \hline 
XNLIV2 \cite{upadhyay2023xnli} & 13 (asm, ben, bho, ell, guj, kan, mar, ory, pan, rus, san...) & PairClassification & s2s & Non-fiction, Fiction, Government & 5010.0 & 80.1 \\
 \hline 
XPQARetrieval \cite{shen2023xpqa} & 13 (ara, cmn, deu, eng, fra, hin, ita, jpn, kor, pol, por...) & Retrieval & s2p & Reviews & 19801.0 & 104.7 \\
 \hline 
XQuADRetrieval \cite{Artetxe:etal:2019} & 12 (arb, deu, ell, eng, hin, ron, rus, spa, tha, tur, vie...) & Retrieval & s2p & Web & 1190.0 & 788.7 \\
 \hline 
XStance \cite{vamvas2020xstance} & 3 (deu, fra, ita) & PairClassification & s2s & Social & 2048.0 & 152.4 \\
 \hline 
YahooAnswersTopicsClassification \cite{NIPS2015_250cf8b5} & 1 (eng) & Classification & s2s & Web & 60000.0 & 346.4 \\
 \hline 
YelpReviewFullClassification \cite{NIPS2015_250cf8b5} & 1 (eng) & Classification & s2s & Reviews & 50000.0 &  \\
 \hline 
YueOpenriceReviewClassification \cite{xiang2019sentiment} & 1 (yue) & Classification & s2s & Reviews & 6161.0 & 173.0 \\
 \hline 
indonli \cite{mahendra-etal-2021-indonli} & 1 (ind) & PairClassification & s2s & Encyclopaedic, Web, News & 2040.0 & 145.9 \\
 \hline 
\end{longtable}
